Guiding Attention for Self-Supervised Learning with Transformers

In this paper, we propose a simple and effective technique to allow for efficient self-supervised learning with bi-directional Transformers. Our approach is motivated by recent studies demonstrating that self-attention patterns in trained models contain a majority of non-linguistic regularities. We propose a computationally efficient auxiliary loss function to guide attention heads to conform to such patterns. Our method is agnostic to the actual pre-training objective and results in faster convergence of models as well as better performance on downstream tasks compared to the baselines, achieving state of the art results in low-resource settings. Surprisingly, we also find that linguistic properties of attention heads are not necessarily correlated with language modeling performance.

==> archive.tex <==
% This paragraph is not entirely supported by our experiments yet
% We find that our attention initialization acts as both an inductive bias and a regularization for the Transformer. Through empirical experiments, we show that our approach enables training large Transformer models in a fraction of the time — for example, we can train a 12-layer Roberta model close to convergence in less than \todo{X} minutes, which is \todo{x\%} of the time taken without our method. Further, the representations learned by our model outperform their corresponding base models on downstream tasks in the GLUE benchmark \karthik{double check this statement} and are competitive with state-of-the-art numbers for the same architecture, despite being much smaller. We also show that our method allows for language model pre-training on low-resource domains without the worry of overfitting. This allows the trained representations to perform better on downstream tasks — e.g. we achieve an \todo{x\%} improvement on the task of named entity recognition (NER) in Filipino. \karthik{double check if task is correct and modify}
% Through empirical experiments, we show that our approach enables training large Transformer models considerably faster — for example, we can train a 16-layer RoBERTa model with competitive performance on the GLUE benchmark in just 4 days on 8 GPUs, while omitting our loss leads to slow or no convergence. We also show that our method allows for language model pre-training on low-resource domains while using less than $4$ GPUs.




%For example, BERT and RoBERTA are trained on $16-64$ TPU chips and $1024$ $32$GB GPUs respectively. Not only does this stymie research in low-resource and low-compute scenarios, but it also hinders research on newer and better pre-train strategies. Comparing different objectives increases the required compute $n-$fold, and researchers are stuck with using domain agnostic hyperparameters and strategies which can often be sub-optimal, given the number of careful design choices needed \cite{liu2020understanding}.

%\note{How training a different language BERT model gives non-trivial performance on English}
%
%\note{Our method can accelerate research on better pre-training strategies}
%
%\note{We are enabling distillation etc.,}
%
%The pretrain-finetune setup for solving natural language understanding and generation tasks has seen a lot of success recently. With models like BERT \cite{devlin2018bert} showing a high correlation between the pretrain loss and downstream performance, a lot of effort has gone into formulating better objectives. However, a large fraction of the improvements tend to increase the number of parameters of an already large model, or require training on commercial-grade GPUs and TPUs which are inaccessible to most of the community. For example, BERT and RoBERTA are trained on $16-64$ TPU chips and $1024$ $32$GB GPUs respectively. Not only does this stymie research in low-resource and low-compute scenarios, but it also hinders research on newer and better pre-train strategies. Comparing different objectives increases the required compute $n-$fold, and researchers are stuck with using domain agnostic hyperparameters and strategies which can often be sub-optimal, given the number of careful design choices needed \cite{liu2020understanding}.
%
%Recent studies investigating self-attention \cite{clark2019does} find recurring patterns like paying attention to the next/prev tokens, or to delimiters like \texttt{[CLS]} which are useful, but don't seem to be linguistically motivated. Indeed we find that these patterns exist in models trained on languages like French and Chinese as well. \note{What happens when these heads are pruned?} More surprisingly, we found that a model trained on French can achieve close to SOTA performance on an English downstream task. This leads us to posit that the structure of attention heads is crucial to pre-training.
%
%Motivated by the observed attention patterns, we add a simple auxiliary loss that can be used with any transformer model and guides the attention heads to exhibit the observed patterns. While this is a simple addition which does not change the memory footprint or the compute time by much \note{report numbers. Around 10\% increase}, it allows large transformer models to converge quickly on Masked Language Modeling (MLM) with as less as $4$ GPUs, while the pure MLM models take a prohibitively long time to train. Moreover, this enables us to train $12-24$ layer models on low-resource domains which have around $1\%$ of the data available in English Wikipedia.
%
%Since our models perform non-trivial tasks even though they have fixed attention patterns, we re-evaluate some recent studies \cite{lin2019open} which claim that individual attention heads can perform linguistically motivated tasks.
%
%Our contribution is three fold
%\begin{enumerate}
%    \item We show that the auxiliary loss allows large models to converge on accessible compute resources ($4-8$ GPUs), and show results on both high and low resource domains
%    \item We show usefulness of the auxiliary loss on different pre-training strategies, which, we hope, will accelerate research in that area
%    \item \note{Our attention analysis calls into question the usefulness of individual attention heads}
%\end{enumerate}


% \begin{table*}
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline \textbf{Model} & \textbf{Variant} & \textbf{MLM Loss} & \textbf{MNLI-m}\\ \hline
% \rowcolor{LightCyan}
% RoBERTa-8 & MLM & 1.75  & 78.3\\ \hline
% \rowcolor{LightCyan}
% RoBERTa-8 & Ours  & 1.74 & 78.2\\ \hline
% RoBERTa-12 & MLM  & 6.32 & 65 \\ \hline
% RoBERTa-12 & Ours  & \textbf{1.73} & \textbf{79.1}\\ \hline
% \rowcolor{LightCyan}
% RoBERTa-16 & MLM  & 6.40 &65\\ \hline
% \rowcolor{LightCyan}
% RoBERTa-16 & Ours  & 1.81 & 79.2\\ \hline
% RoBERTa-Uniq-12 & MLM  & 1.89 & 78.1\\ \hline
% Only-Attention-24 & Ours & 1.90 & 78.0\\ \hline
% \rowcolor{LightCyan}
% Only-Attention-48 & MLM & 7.7 & 65\\ \hline
% \rowcolor{LightCyan}
% Only-Attention-48 & Ours  & 2.4 &  75.1\\ \hline
% ELMo & - & - & 74.1\\ \hline
% Only-Finetune & - & - & 61.0\\ \hline
% \end{tabular}
% \caption{Pre-training on English Wikipedia \note{Will report GLUE}}
% \label{table:wiki_results}
% \end{table*}



% \begin{table*}
% \centering
% \begin{tabular}{|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{2}{c|}{\textbf{MLM Loss}} & \multicolumn{2}{c|}{\textbf{MNLI-m}} \\
% \cline{2-3}\cline{4-5}
% %  & \multicolumn{2}{c|}{Value} & & \multicolumn{2}{c|}{Value} & \\
%  & \textbf{Base} & \textbf{+Attn-Init} & \textbf{Base} & \textbf{+Attn-Init} \\ \hline
% % \cline{2-3}\cline{5-6}
% %  & B1 & B2 & & C1 & C2 & \\
% RoBERTa-8 & 1.75 & \textbf{1.74} & \textbf{78.3} & 78.2 \\ \hline
% RoBERTa-12 & 6.32 & \textbf{1.73} & 65 & \textbf{79.1} \\ \hline
% RoBERTa-12 (350000) & 6.32 & \textbf{1.73} & 65 & \textbf{77.6/78.9} \\ \hline
% RoBERTa-16 & 6.40 & \textbf{1.81} & 65 & \textbf{78.7/79.6} \\ \hline
% RoBERTa-AH-12 & \textbf{1.89} & 1.90 & \textbf{78.1} & 78.0 \\ \hline
% RoBERTa-AH-24 & 7.7 & \textbf{2.4} & 65 & \textbf{75.1} \\ \hline
% ELMo \cite{peters2018deep} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{74.1} \\ \hline
% Only-Finetune & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{61.0} \\ \hline
% % etc. ...
% \end{tabular}
% \caption{Pre-training on English Wikipedia \note{Will report GLUE}}
% \label{table:wiki_results}
% \end{table*}



\section{Approach}

As mentioned in Section~\ref{sec:related_work}, several studies~\cite{clark2019does,kovaleva2019revealing} have demonstrated that Transformers trained with the masked language modeling (MLM) objective exhibit simple patterns~\ref{fig:attentionpatterns} in their self-attention layers (e.g. attending to delimiter tokens). These patterns also seem to be consistent across models pre-trained on different languages, and fine-tuned on varied downstream tasks. However, since these patterns do not carry much linguistic signal, we hypothesize that it should be possible to induce them without requiring multiple days of training. While all the desired patterns are mathematically simple to express, the varying distribution of inputs makes it difficult to guide them to specific patterns without any training. This also allows the procedure to be model agnostic. To satisfy these desiderata, we propose to use auxiliary losses on the intermediate attention layers to guide them towards desired patterns.

% \[\textrm{\texttt{next}} = \begin{bmatrix}
% 0 & 1 & 0 \\
% 0 & 0 & 1 \\
% \frac{1}{3} & \frac{1}{3} & \frac{1}{3}
% \end{bmatrix} \quad \textrm{\texttt{prev}} = \begin{bmatrix}
% \frac{1}{3} & \frac{1}{3} & \frac{1}{3} \\
% 1 & 0 & 0 \\
% 0 & 1 & 0
% \end{bmatrix} \]


\section{Results}

% \note{Experiments in progress. But trends are similar}

% \note{VilBERT author's note that domain similarity plays a crucial role}

% \begin{enumerate}
%     \item Motivate usage of large models even for low-resource tasks (domain mismatch, can be used with regularization, continual learning, and just better empirical performance)
% \end{enumerate}

% Loss curves in figure \ref{fig:tempfilipino} show that convergence is hard for pure MLM models but not a problem for our models.


% \begin{figure}[ht]
% \vskip 0.2in
% \begin{center}
% \centerline{\includegraphics[width=\columnwidth]{Figures/temp_filipino.png}}
% \caption{Loss Curves}
% \label{fig:tempfilipino}
% \end{center}
% \vskip -0.2in
% \end{figure}

\begin{table*}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{Base Model}} & \multicolumn{2}{c|}{\textbf{MLM Loss}} &
\multicolumn{2}{c|}{\textbf{MLM Valid Loss}} &\multicolumn{2}{c|}{\textbf{FSST-2}} \\
\cline{2-3}\cline{4-5}\cline{6-7}
%  & \multicolumn{2}{c|}{Value} & & \multicolumn{2}{c|}{Value} & \\
 & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} \\ \hline
% \cline{2-3}\cline{5-6}
%  & B1 & B2 & & C1 & C2 & \\
RoBERTa-8 & 3.1 & 0.74 & 3.22 & 0.99 & 74.9/74.1 & 76.7/75.6 \\ \hline
RoBERTa-12 & 5.04 & 0.66 & 5.06 & 0.97 & 75.3/74.1 & 75.9/74.6 \\ \hline
RoBERTa-16 & 5.18 & 0.63 & 5.05 & 0.82 & 74.9/74.1 & 77.2/75.5 \\ \hline
BERT-Base-Tagalog & \multicolumn{2}{c|}{0.09} & \multicolumn{2}{c|}{1.74} & \multicolumn{2}{c|}{74.76} \\ \hline
% etc. ...
\end{tabular}
\caption{Filipino}
\label{table:filipino}
\end{table*}


\begin{table*}
\centering
\begin{tabular}{|l|c|c|c|c|}
\hline 
\multirow{2}{*}{\textbf{Model}} & \multicolumn{2}{c|}{\textbf{Without Distractor}} & \multicolumn{2}{c|}{\textbf{With distractor}} \\
\cline{2-3}\cline{4-5}
 & \textbf{Max} & \textbf{Mean} & \textbf{Max} & \textbf{Mean} \\ \hline
RoBERTa-Base \cite{liu2019roberta} & 0.999 & 0.068 & 0.998 & 0.067 \\ \hline
% RoBERTa-Attn ($\lambda=1/2$) & 0.674 &  0.047 & 0.704 & 0.047 \\ \hline
RoBERTa-12-AUX ($\lambda=1/2$) & 0.841 &  0.041 & 0.836  & 0.047  \\ \hline
RoBERTa-Attn ($\lambda=1$)  & 0.0  & 0.0 & 0.0 & 0.0 \\ \hline
Randomly Initialized  & 0.296 & 0.16 & 0.452 & 0.16 \\ \hline
% Nearest Mention \note{Should we have this here?}  & 1.0 & - & 1.0 & - \\ \hline
\end{tabular}
\caption{Coreference Resolution}
\label{table:coreference}
\end{table*}


%\begin{table*}
%\centering
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multirow{2}{*}{\textbf{Base Model}} & \multicolumn{2}{c|}{\textbf{MLM Loss}} & \multicolumn{2}{c|}{\textbf{MLM Valid Loss}} & \multicolumn{2}{c|}{\textbf{MNLI-m}} \\
%\cline{2-3}\cline{4-5}\cline{6-7}
%%  & \multicolumn{2}{c|}{Value} & & \multicolumn{2}{c|}{Value} & \\
% & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} \\ \hline
%% \cline{2-3}\cline{5-6}
%%  & B1 & B2 & & C1 & C2 & \\
%RoBERTa-8 & 1.75 & \textbf{1.74} & 2.41 & 2.43 & \textbf{78.3} & 78.2 \\ \hline
%RoBERTa-12 & 1.86 & \textbf{1.73} & 2.47 & 2.29 & 78.9 & \textbf{79.0} \\ \hline
%% RoBERTa-12 (350000) & \note{6.32} & \textbf{1.73} & \note{7} & \note{2.5} & 65 & \textbf{77.6/78.9} \\ \hline
%RoBERTa-16 & 6.40 & \textbf{1.81} & 7.28 & 2.46 & 65 & \textbf{78.7/79.6} \\ \hline
%% RoBERTa-AH-12 & \textbf{1.89} & 1.90 & & & \textbf{78.1} & 78.0 \\ \hline
%% RoBERTa-AH-24 & 7.7 & \textbf{2.4} & & & 65 & \textbf{75.1} \\ \hline \hline
%ELMo \cite{peters2018deep} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{74.1} \\ \hline
%RoBERTa \cite{liu2019roberta} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{84.7} \\ \hline
%% Only-Finetune & \multicolumn{2}{c|}{-} &\multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{61.0} \\ \hline
%% etc. ...
%\end{tabular}
%\caption{Pre-training on English Wikipedia \note{Will report GLUE}}
%\label{table:wiki_results}
%\end{table*}


\karthik{The table below (in tex file) leads to some compile errors. But we need something like that for downstream results.}
% \begin{table}[t]
% \centering
% \begin{tabular}{c c c c c}
% Language & Task & Metric & \multicolumn{2}{c}{Result} \\  \cmidrule(lr){4-5}
% & & & MLM & AG \\ \cmidrule
% &c  & & & & \\ \bottomrule
% \end{tabular}
% \caption{Downstream results\karthik{fill in numbers}}
% \label{table:downstream}
% \end{table}


% \begin{table*}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{2}{c|}{\textbf{MLM Loss}} &
% \multicolumn{2}{c|}{\textbf{MLM Valid Loss}} &\multicolumn{2}{c|}{\textbf{FSST-2}} \\
% \cline{2-3}\cline{4-5}\cline{6-7}
% %  & \multicolumn{2}{c|}{Value} & & \multicolumn{2}{c|}{Value} & \\
% & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} \\ \hline
% % \cline{2-3}\cline{5-6}
% %  & B1 & B2 & & C1 & C2 & \\
% RoBERTa-8 & 3.1 & \textbf{0.74} & 3.22 & \textbf{0.99} & 74.1 & \textbf{75.6}* \\ \hline
% RoBERTa-12 & 5.04 & \textbf{0.66} & 5.06 & \textbf{0.97} & 74.1 & \textbf{74.6} \\ \hline
% RoBERTa-16 & 5.18 & \textbf{0.63} & 5.05 & \textbf{0.82} & 74.1 & \textbf{75.5} \\ \hline
% BERT-Base-Tagalog & \multicolumn{2}{c|}{0.09} & \multicolumn{2}{c|}{1.74} & \multicolumn{2}{c|}{74.76} \\ \hline
% % etc. ...
% \end{tabular}
% \caption{Filipino}
% \label{table:filipino}
% \end{table*}

% \begin{table*}
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% \multirow{2}{*}{\textbf{Base Model}} & \multicolumn{2}{c|}{\textbf{Train Loss}} &
% \multicolumn{2}{c|}{\textbf{Valid Loss}} &\multicolumn{2}{c|}{\textbf{NER}} \\
% \cline{2-3}\cline{4-5}\cline{6-7}
% %  & \multicolumn{2}{c|}{Value} & & \multicolumn{2}{c|}{Value} & \\
% & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} & \textbf{MLM} & \textbf{AUX} \\ \hline
% % \cline{2-3}\cline{5-6}
% %  & B1 & B2 & & C1 & C2 & \\
% RoBERTa-8 & 3.44 & \textbf{3.31} & 4.06 & \textbf{3.93} & 64.6 & \textbf{66.7} \\ \hline
% RoBERTa-12 & 6.24 & \textbf{3.23} & 6.74 & \textbf{3.88} & 51.5 & \textbf{67.9} \\ \hline
% % RoBERTa-16 & 5.18 & 0.63 & 5.05 & 0.82 & 74.9/74.1 & 77.2/75.5 \\ \hline
% E-MBERT & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{-} & \multicolumn{2}{c|}{72.8*} \\ \hline
% % etc. ...
% \end{tabular}
% \caption{Oromo}
% \label{table:oromo}
% \end{table*}




% \begin{table*}
% \centering
% \begin{tabular}{|l|c|c|c|}
% \hline 
% \textbf{Model} & \textbf{MLM Validation} & \textbf{Max} & \textbf{Mean} \\ \hline
% RoBERTa-Base \cite{liu2019roberta} & - & 0.998 & 0.067 \\ \hline
% % RoBERTa-Attn ($\lambda=1/2$) & 0.674 &  0.047 & 0.704 & 0.047 \\ \hline
% RoBERTa-AUX ($\lambda=1/2$) & 2.29 & 0.836  & 0.047  \\ \hline
% RoBERTa-AUX ($\lambda=1$) & 2.31 & 0.0 & 0.0 \\ \hline
% Randomly Initialized & - & 0.266 & 0.154 \\ \hline
% % Nearest Mention \note{Should we have this here?}  & 1.0 & - & 1.0 & - \\ \hline
% \end{tabular}
% \caption{Coreference Resolution}
% \label{table:coreference}
% \end{table*}

% \paragraph{Attention Heavy Transformers}
% We also experiment with a variant of standard Transformers proposed by \cite{press2019improving}, who showed that alternating feed forward layers and self-attention layers is not the most optimal layout. We use $12$ and $24$ layer models with multiple attention layers stacked together before a feed forward layer. Specifically, we train models whose layers are given by the regular expression $(AAAF)^+$ instead of the usual $(AFAF)^+$, where $A$ is a self-attention layer, $F$ is a feed-forward layer, and $^+$ is the kleene plus operator. This can be interpreted as a replacement of every alternate feedforward layer with an attention layer. These models have lesser parameters than their counterparts because each self-attention layer has half the parameters in feed-forward layers. We call these models RoBERTa-AH-12 and RoBERTa-AH-24, where AH stands for Attention-Heavy. 

%\paragraph{Best performing AUX variants} RoBERTa-AG is surprisingly robust to hyperparameters. Other than $\alpha$, which depends on the model size, the same design choices perform well on all model sizes and domains.  We use a $\lambda$ of half, which amounts to modifying half the heads in each layer. One head each is modified with the \texttt{[Next]} and \texttt{[Prev]} patterns, and $(\lambda h-2)$ heads are modified with \texttt{[First]}. We observed that adding \texttt{[Delim]} led to no significant change in performance and \texttt{[Period]} led to small decrease. RoBERTa-MLM on the other hand was very sensitive to the number of warmup steps and the learning rate, and the best performing hyperparameters for each model is reported in the appendix \note{appendix}.


We compare the language modeling and downstream performance of the models with and without our auxiliary loss in Table \ref{table:wiki_results}, and this makes our comparisons hardware independent. Each model is trained for $10$ epochs or 4 days\footnote{RoBERT-8 ran for $10$ epochs, RoBERTa-12 for $8.2$, and RoBERTa-16 for $4.3$}, whichever is lesser, on 8 NVIDIA Tesla P40 GPUs.


As seen from the GLUE scores, this convergence also translates to good downstream performance. With just 3 days of training on 8 GPUs \note{which is a fraction of compute}, RoBERTa-12-Attn is able to achieve an MNLI score of $79.1$. We emphasize that these scores are not comparable to SOTA models which are trained on more data, up to $8$ times more epochs, and on more compute. To show that the scores are non-trivial, we include ELMo's \cite{peters2018deep} scores. Table \ref{table:wiki_results} summarizes our results. \textit{Only-Finetune} represents a model which is finetuned on GLUE without any pre-training \cite{kovaleva2019revealing}. 


% It has been noted in experiments \note{Need to cite \href{https://github.com/pytorch/fairseq/blob/master/examples/roberta/README.pretraining.md}{link}} that large batch sizes or low learning rates are required to train transformer models. BERT uses a batch size of $256$. Both \cite{liu2019roberta} and \cite{raffel2019exploring} note that increasing the batch size from $256$ to $1024$ or $2048$ leads to improved performance. But most of these training regimes are inaccessible with a compute of $4$-$8$ GPUs.

% RoBERTa also uses a lot of tricks to ensure convergence, like a warmup period for the learning rate and layer normalization, and some recent studies \cite{xiong2020layer} have questioned the instability of models in their absence.
% https://stackoverflow.com/questions/32291026/latex-table-multiple-row-and-multiple-column


% The rate of convergence with respect to the number of steps trained is always faster for our models. Figure \ref{fig:rob8rob12curves} shows the loss curves for RoBERTa-8 and RoBERTa-12. Additional loss curves are reported in the appendix \note{Appendix}. While RoBERTa-8 and Only-Attention-24 are able to converge (albeit slowly) when using only the MLM loss, the larger models train very slowly, thus performing as bad as random on downstream tasks. We emphasize that while our scores are not comparable to state of the art scores because we train on a fraction of compute and total number of epochs, we can still match or exceed the performance of models like  \note{Only on MNLI though, check SST-2 again}. \note{After the runs with 256 batch size are complete, show that attn\_init and mlm converge to the same loss and downstream performance}.


\begin{table*}[t]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccc}\toprule
\multirow{2}{*}{\textbf{Language}} & \multirow{2}{*}{\textbf{Task}} & \multicolumn{2}{c }{\textbf{RoBERTa-8}} &\multicolumn{2}{c }{\textbf{RoBERTa-12}} & \multicolumn{2}{c }{\textbf{RoBERTa-16}} & \multicolumn{2}{c }{\textbf{Literature}} \\ \cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8} \cmidrule(lr){9-10}  
%  & \multicolumn{2}{c }{\textbf{Train}}  & \multicolumn{2}{c }{\textbf{Validation}} & \multicolumn{2}{c }{\textbf{Train}}  & \multicolumn{2}{c }{\textbf{Validation}}& \multicolumn{2}{c }{\textbf{Train}}  & \multicolumn{2}{c }{\textbf{Validation}}\\ \cmidrule(lr){2-3} \cmidrule(lr){4-5}  \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
 & & MLM & AG & MLM & AG  &  MLM & AG & Model & Score \\ \midrule
%  &  MLM & AG & MLM & AG  &  MLM & AG & MLM & AG  &  MLM & AG & MLM & AG \\ \midrule
\multirow{4}{*}{\textbf{English}} & MNLI-m & 78.8 & \textbf{79.1} & 78.9 & \textbf{79.0} & 69.7 & \textbf{79.6} & \multirow{4}{*}{BERT$_{\textrm{BASE}}$~\cite{devlin2018bert}} & 84.6$^\star$ \\
& MNLI-mm & 77.6 & \textbf{77.7} & 77.6 & \textbf{78.9} & 68.8 & \textbf{78.7} &  & 83.4$^\star$ \\
& QNLI & 84.3 & \textbf{84.6} & 86.1 & \textbf{86.8} & 72.0 & \textbf{84.4} &  & 90.5$^\star$ \\
& QQP & \textbf{69.1/88.1} & 68.3/87.5 & 68.4/87.7 & \textbf{68.9/87.8} & 58.2/84.9 & \textbf{68.5/87.8} &  & 71.2/89.2$^\star$ \\ \midrule
\multirow{1}{*}{\textbf{Filipono}} & Sentiment & 74.1 & \textbf{75.6}$^\star$ & 74.1 & \textbf{74.6} & 74.1 & \textbf{75.5} & BERT~\cite{cruz2020establishing} & 74.8 \\ \midrule
\multirow{1}{*}{\textbf{Oromo}} & NER & 64.6 & \textbf{66.7} & 51.5 & \textbf{67.9} & - & - & E-MBERT~\cite{wang2020extending} & 72.8$^\star$  \\
\bottomrule
\end{tabular}
}
\caption{Main table on downstream tasks}
\label{table:downstream}
\end{table*}


\paragraph{Filipino} As shown in table \ref{table:downstream}, our AG models outperform the MLM variants on all model sizes. Given that the dataset for pre-training is much smaller than English, we follow \cite{devlin2018bert} and train all models for $40$ epochs and within one day. Since the current SOTA for this dataset~\cite{cruz2019evaluating} is a BERT model rather than RoBERTa, to ensure fair comparison we use our auxiliary loss with BERT instead of RoBERTa. The results in table \ref{table:filipino} show that for all model sizes, the AUX model outperforms the MLM model on speed of convergence, final train and validation loss, and downstream score on sentiment classification. Additionally, our best performing model beats~\cite{cruz2019evaluating} by almost $1$ point, even though the latter was trained on a TPU for over a day.


\paragraph{Oromo} Given the small dataset size when compared to other settings, we train the MLM and AUX variants of RoBERTa-8 and RoBERTa-12, and omit the 16 layer variant to avoid overfitting. The AUX models outperform the MLM models on all metrics and achieve significantly better scores on the NER task. We believe that better performance of our AUX models in Oromo can in part be attributed to the regularizing effect of guiding attention, which constraints the parameters. We also compare against E-MBERT~\cite{wang2020extending}, which is a BERT model leveraging resources from over 104 languages. While the comparison is not fair because of the orders of magnitude more data that it is trained on, we include it for reference.


\begin{table}
\centering
\resizebox{1\columnwidth}{!}{
\begin{tabular}{c c c c c c}
\toprule
\multirow{2}{*}{\textbf{Language}} & \multicolumn{2}{c }{\textbf{LM}} & \multicolumn{3}{c }{\textbf{Downstream task}} \\ \cmidrule(lr){2-3} \cmidrule(lr){4-6}  
 & \textbf{Train size} & \textbf{Valid size} & \textbf{Task} & \textbf{\# instances} & \textbf{Evaluation Metric} \\ \midrule

English & 2116M & 1\% & MNLI, QNLI, QQP & 3k-390k & Accuracy/F-1\\
Filipino & 36M & 10\% & Sentiment classification & 10k & Accuracy\\ 
Oromo & 4.6M & 3\% & NER & 1k & F-1\\ \bottomrule
\end{tabular}
}
\caption{Dataset statistics for pre-training and finetuning tasks on English, Filipino, and Oromo}
\label{table:dataset_stats_1}
\end{table}

\begin{table}
\centering
\begin{tabular}{c c c}
\toprule
\textbf{Model} & \textbf{Final Loss} & \textbf{Average Loss} \\ \midrule 

ELECTRA & 0.27  & 0.32 \\
ELECTRA-AG & \textbf{0.10}  & \textbf{0.15} \\ \bottomrule
\end{tabular}
\caption{ELECTRA. \karthik{fill details} \karthik{Transpose this table to make it similar to other tables?}}
\label{table:electra}
\end{table}
